Non-Orthogonal Multiple Access for FSO Backhauling

We consider a free space optical (FSO) backhauling system which consists of two base stations (BSs) and one central unit (CU). We propose to employ non-orthogonal multiple access (NOMA) for FSO backhauling where both BSs transmit at the same time and in the same frequency band to the same photodetector at the CU. We develop a dynamic NOMA scheme which determines the optimal decoding order as a function of the channel state information at the CU and the quality of service requirements of the BSs, such that the outage probabilities of both BSs are jointly minimized. Moreover, we analyze the performance of the proposed NOMA scheme in terms of the outage probability over Gamma-Gamma FSO turbulence channels. We further derive closed-form expressions for the outage probability for the high signal-to-noise ratio regime. Our simulation results confirm the analytical derivations and reveal that the proposed dynamic NOMA scheme significantly outperforms orthogonal transmission and existing NOMA schemes.

==> Fig/Outage/Outage.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA Fixed NOMA}%
\psfrag{013}[cl][cl]{\matlabtextA Dynamic NOMA in [11]}%
\psfrag{014}[cl][cl]{\matlabtextA OMA}%
\psfrag{015}[cl][cl]{\matlabtextA Proposed NOMA (Numerical)}%
\psfrag{016}[cl][cl]{\matlabtextA Proposed NOMA (Simulation)}%
\psfrag{017}[cl][cl]{\matlabtextA Lower Bound}%
\psfrag{018}[cl][cl]{\matlabtextA BS$_2$}%
\psfrag{019}[cl][cl]{\matlabtextA BS$_1$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{020}[bc][bc]{\matlabtextB Outage Probability}%
\psfrag{021}[tc][tc]{\matlabtextB $P$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{009}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>

==> Fig/Outage2/Outage.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA Asymptotic}%
\psfrag{013}[cl][cl]{\matlabtextA Numerical}%
\psfrag{014}[cl][cl]{\matlabtextA Simulation}%
\psfrag{015}[cl][cl]{\matlabtextA $\kappa=20\times 10^{-3}$}%
\psfrag{016}[cl][cl]{\matlabtextA $\kappa=0.43\times 10^{-3}$}%
\psfrag{017}[cl][cl]{\matlabtextA $\epsilon=\{-10^{-1},-10^{-3},10^{-3},10^{-1}\}$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{018}[bc][bc]{\matlabtextB Outage Probability}%
\psfrag{019}[tc][tc]{\matlabtextB $P$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $\matlabfragNegXTick 20$}%
\psfrag{001}[ct][ct]{\matlabtextC $\matlabfragNegXTick 10$}%
\psfrag{002}[ct][ct]{\matlabtextC $0$}%
\psfrag{003}[ct][ct]{\matlabtextC $10$}%
\psfrag{004}[ct][ct]{\matlabtextC $20$}%
\psfrag{005}[ct][ct]{\matlabtextC $30$}%
\psfrag{006}[ct][ct]{\matlabtextC $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{007}[rc][rc]{\matlabtextC $10^{-4}$}%
\psfrag{008}[rc][rc]{\matlabtextC $10^{-3}$}%
\psfrag{009}[rc][rc]{\matlabtextC $10^{-2}$}%
\psfrag{010}[rc][rc]{\matlabtextC $10^{-1}$}%
\psfrag{011}[rc][rc]{\matlabtextC $10^{0}$}%
%
%% </ytick>
